Vast TVB parameter space exploration: A Modular Framework for Accelerating the Multi-Scale Simulation of Human Brain Dynamics

Global neural dynamics emerge from multi-scale brain structures, with neurons communicating through synapses to form transiently communicating networks. Network activity arises from intercellular communication that depends on the structure of connectome tracts and local connection, intracellular signalling cascades, and the extracellular molecular milieu that regulate cellular properties. Multi-scale models of brain function have begun to directly link the emergence of global brain dynamics in conscious and unconscious brain states to microscopic changes at the level of cells. In particular, AdEx mean-field models representing statistical properties of local populations of neurons have been connected following human tractography data to represent multi-scale neural phenomena in simulations using The Virtual Brain (TVB). While mean-field models can be run on personal computers for short simulations, or in parallel on high-performance computing (HPC) architectures for longer simulations and parameter scans, the computational burden remains high and vast areas of the parameter space remain unexplored. In this work, we report that our TVB-HPC framework, a modular set of methods used here to implement the TVB-AdEx model for GPU and analyze emergent dynamics, notably accelerates simulations and substantially reduces computational resource requirements. The framework preserves the stability and robustness of the TVB-AdEx model, thus facilitating finer resolution exploration of vast parameter spaces as well as longer simulations previously near impossible to perform. Given that simulation and analysis toolkits are made public as open-source packages, our framework serves as a template onto which other models can be easily scripted and personalized datasets can be used for studies of inter-individual variability of parameters related to functional brain dynamics.

==> biblio.tex <==
@article{goldman2023asynchronous,
  title={Asynchronous and slow-wave oscillatory states in connectome-based models of mouse, monkey and human cerebral cortex},
  author={Goldman, Jennifer S and Sacha, Maria and kusch, lionel and Destexhe, Alain},
  journal={bioRxiv},
  pages={2023--08},
  year={2023},
  publisher={Cold Spring Harbor Laboratory}
}

@article{schirner2018inferring,
  title={Inferring multi-scale neural mechanisms with brain network modelling},
  author={Schirner, Michael and McIntosh, Anthony Randal and Jirsa, Viktor and Deco, Gustavo and Ritter, Petra},
  journal={elife},
  volume={7},
  pages={e28927},
  year={2018},
  publisher={eLife Sciences Publications, Ltd}
}

@article{goldman2019bridging,
  title={Bridging single neuron dynamics to global brain states},
  author={Goldman, Jennifer S and Tort-Colet, N{\'u}ria and Di Volo, Matteo and Susin, Eduarda and Bout{\'e}, Jules and Dali, Melissa and Carlu, Mallory and Nghiem, Trang-Anh and G{\'o}rski, Tomasz and Destexhe, Alain},
  journal={Frontiers in systems neuroscience},
  volume={13},
  pages={75},
  year={2019},
  publisher={Frontiers}
}

@article{zerlaut2018modeling,
  title={Modeling mesoscopic cortical dynamics using a mean-field model of conductance-based networks of adaptive exponential integrate-and-fire neurons},
  author={Zerlaut, Yann and Chemla, Sandrine and Chavane, Frederic and Destexhe, Alain},
  journal={Journal of computational neuroscience},
  volume={44},
  number={1},
  pages={45--61},
  year={2018},
  publisher={Springer}
}

@article{Sanzleon2013,
abstract = {We present TheVirtualBrain (TVB), a neuroinformatics platform for full brain network simulations using biologically realistic connectivity. This simulation environment enables the model-based inference of neurophysiological mechanisms across different brain scales that underlie the generation of macroscopic neuroimaging signals including functional MRI (fMRI), EEG and MEG. Researchers from different backgrounds can benefit from an integrative software platform including a supporting framework for data management (generation, organization, storage, integration and sharing) and a simulation core written in Python. TVB allows the reproduction and evaluation of personalized configurations of the brain by using individual subject data. This personalization facilitates an exploration of the consequences of pathological changes in the system, permitting to investigate potential ways to counteract such unfavorable processes. The architecture of TVB supports interaction with MATLAB packages, for example, the well known Brain Connectivity Toolbox. TVB can be used in a client-server configuration, such that it can be remotely accessed through the Internet thanks to its web-based HTML5, JS and WebGL graphical user interface. TVB is also accessible as a standalone cross-platform Python library and application, and users can interact with the scientific core through the scripting interface IDLE, enabling easy modeling, development and debugging of the scientific kernel. This second interface makes TVB extensible by combining it with other libraries and modules developed by the Python scientific community. In this article, we describe the theoretical background and foundations that led to the development of TVB, the architecture and features of its major software components as well as potential neuroscience applications. {\textcopyright} 2013 Sanz_leon, Knock, Woodman, Domide, Mersmann, Mcintosh and Jirsa.},
author = {Sanzleon, Paula and Knock, Stuart A. and Woodman, M. Marmaduke and Domide, Lia and Mersmann, Jochen and Mcintosh, Anthony R. and Jirsa, Viktor},
doi = {10.3389/fninf.2013.00010},
file = {:home/myguy/Downloads/fninf-07-00010.pdf:pdf},
issn = {16625196},
journal = {Frontiers in Neuroinformatics},
keywords = {Connectivity,Connectome,Full-brain network model,GPUs,Large-scale simulation,Neural field,Neural mass,Python,Time delays,Virtual brain,Web platform},
number = {MAY},
title = {{The virtual brain: A simulator of primate brain network dynamics}},
volume = {7},
year = {2013}
}

@article{NeuroML,
doi = {10.1371/journal.pcbi.1000815},
author = {Gleeson, Padraig AND Crook, Sharon AND Cannon, Robert C. AND Hines, Michael L. AND Billings, Guy O. AND Farinella, Matteo AND Morse, Thomas M. AND Davison, Andrew P. AND Ray, Subhasis AND Bhalla, Upinder S. AND Barnes, Simon R. AND Dimitrova, Yoana D. AND Silver, R. Angus},
journal = {PLOS Computational Biology},
publisher = {Public Library of Science},
title = {NeuroML: A Language for Describing Data Driven Models of Neurons and Networks with a High Degree of Biological Detail},
year = {2010},
month = {06},
volume = {6},
url = {https://doi.org/10.1371/journal.pcbi.1000815},
pages = {1-19},
abstract = {Biologically detailed single neuron and network models are important for understanding how ion channels, synapses and anatomical connectivity underlie the complex electrical behavior of the brain. While neuronal simulators such as NEURON, GENESIS, MOOSE, NEST, and PSICS facilitate the development of these data-driven neuronal models, the specialized languages they employ are generally not interoperable, limiting model accessibility and preventing reuse of model components and cross-simulator validation. To overcome these problems we have used an Open Source software approach to develop NeuroML, a neuronal model description language based on XML (Extensible Markup Language). This enables these detailed models and their components to be defined in a standalone form, allowing them to be used across multiple simulators and archived in a standardized format. Here we describe the structure of NeuroML and demonstrate its scope by converting into NeuroML models of a number of different voltage- and ligand-gated conductances, models of electrical coupling, synaptic transmission and short-term plasticity, together with morphologically detailed models of individual neurons. We have also used these NeuroML-based components to develop an highly detailed cortical network model. NeuroML-based model descriptions were validated by demonstrating similar model behavior across five independently developed simulators. Although our results confirm that simulations run on different simulators converge, they reveal limits to model interoperability, by showing that for some models convergence only occurs at high levels of spatial and temporal discretisation, when the computational overhead is high. Our development of NeuroML as a common description language for biophysically detailed neuronal and network models enables interoperability across multiple simulation environments, thereby improving model transparency, accessibility and reuse in computational neuroscience.},
number = {6},

}

@article{PyLems,
abstract = {NeuroML is an XML-based model description language, which provides a powerful common data format for defining and exchanging models of neurons and neuronal networks. In the latest version of NeuroML, the structure and behavior of ion channel, synapse, cell, and network model descriptions are based on underlying definitions provided in LEMS, a domain-independent language for expressing hierarchical mathematical models of physical entities. While declarative approaches for describing models have led to greater exchange of model elements among software tools in computational neuroscience, a frequent criticism of XML-based languages is that they are difficult to work with directly. Here we describe two Application Programming Interfaces (APIs) written in Python (<ext-link ext-link-type="uri" xlink:href="http://www.python.org" xmlns:xlink="http://www.w3.org/1999/xlink">http://www.python.org</ext-link>), which simplify the process of developing and modifying models expressed in NeuroML and LEMS. The libNeuroML API provides a Python object model with a direct mapping to all NeuroML concepts defined by the NeuroML Schema, which facilitates reading and writing the XML equivalents. In addition, it offers a memory-efficient, array-based internal representation, which is useful for handling large-scale connectomics data. The libNeuroML API also includes support for performing common operations that are required when working with NeuroML documents. Access to the LEMS data model is provided by the PyLEMS API, which provides a Python implementation of the LEMS language, including the ability to simulate most models expressed in LEMS. Together, libNeuroML and PyLEMS provide a comprehensive solution for interacting with NeuroML models in a Python environment.},
author = {Vella, Michael and Cannon, Robert C and Crook, Sharon and Davison, Andrew P and Ganapathy, Gautham and Robinson, Hugh P C and Silver, R Angus and Gleeson, Padraig},
doi = {10.3389/fninf.2014.00038},
issn = {1662-5196},
journal = {Frontiers in Neuroinformatics},
pages = {38},
title = {{libNeuroML and PyLEMS: using Python to combine procedural and declarative modeling approaches in computational neuroscience}},
url = {https://www.frontiersin.org/article/10.3389/fninf.2014.00038},
volume = {8},
year = {2014}
}

@ARTICLE{LEMS,
  
AUTHOR={Cannon, Robert C. and Gleeson, Padraig and Crook, Sharon and Ganapathy, Gautham and Marin, Boris and Piasini, Eugenio and Silver, R. Angus},   
	 
TITLE={LEMS: a language for expressing complex biological models in concise and hierarchical form and its use in underpinning NeuroML 2},      
	
JOURNAL={Frontiers in Neuroinformatics},      
	
VOLUME={8},      

PAGES={79},     
	
YEAR={2014},      
	  
URL={https://www.frontiersin.org/article/10.3389/fninf.2014.00079},       
	
DOI={10.3389/fninf.2014.00079},      
	
ISSN={1662-5196},   
   
ABSTRACT={Computational models are increasingly important for studying complex neurophysiological systems. As scientific tools, it is essential that such models can be reproduced and critically evaluated by a range of scientists. However, published models are currently implemented using a diverse set of modeling approaches, simulation tools, and computer languages making them inaccessible and difficult to reproduce. Models also typically contain concepts that are tightly linked to domain-specific simulators, or depend on knowledge that is described exclusively in text-based documentation. To address these issues we have developed a compact, hierarchical, XML-based language called LEMS (Low Entropy Model Specification), that can define the structure and dynamics of a wide range of biological models in a fully machine readable format. We describe how LEMS underpins the latest version of NeuroML and show that this framework can define models of ion channels, synapses, neurons and networks. Unit handling, often a source of error when reusing models, is built into the core of the language by specifying physical quantities in models in terms of the base dimensions. We show how LEMS, together with the open source Java and Python based libraries we have developed, facilitates the generation of scripts for multiple neuronal simulators and provides a route for simulator free code generation. We establish that LEMS can be used to define models from systems biology and map them to neuroscience-domain specific simulators, enabling models to be shared between these traditionally separate disciplines. LEMS and NeuroML 2 provide a new, comprehensive framework for defining computational models of neuronal and other biological systems in a machine readable format, making them more reproducible and increasing the transparency and accessibility of their underlying structure and properties.}
}

@misc{NumbaWeb,
author = {Numba},
title = {{Creating NumPy universal functions}},
url = {https://numba.pydata.org/numba-doc/latest/user/vectorize.html},
year = {2012}
}

@inproceedings{Numba,
author = {Lam, Siu Kwan and Pitrou, Antoine and Seibert, Stanley},
title = {Numba: A LLVM-Based Python JIT Compiler},
year = {2015},
isbn = {9781450340052},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2833157.2833162},
doi = {10.1145/2833157.2833162},
abstract = {Dynamic, interpreted languages, like Python, are attractive for domain-experts and scientists experimenting with new ideas. However, the performance of the interpreter is often a barrier when scaling to larger data sets. This paper presents a just-in-time compiler for Python that focuses in scientific and array-oriented computing. Starting with the simple syntax of Python, Numba compiles a subset of the language into efficient machine code that is comparable in performance to a traditional compiled language. In addition, we share our experience in building a JIT compiler using LLVM[1].},
booktitle = {Proceedings of the Second Workshop on the LLVM Compiler Infrastructure in HPC},
articleno = {7},
numpages = {6},
keywords = {Python, compiler, LLVM},
location = {Austin, Texas},
series = {LLVM '15}
}

@article{NeuroML,
abstract = {Computational models are increasingly important for studying complex neurophysiological systems. As scientific tools, it is essential that such models can be reproduced and critically evaluated by a range of scientists. However, published models are currently implemented using a diverse set of modeling approaches, simulation tools, and computer languages making them inaccessible and difficult to reproduce. Models also typically contain concepts that are tightly linked to domain-specific simulators, or depend on knowledge that is described exclusively in text-based documentation. To address these issues we have developed a compact, hierarchical, XML-based language called LEMS (Low Entropy Model Specification), that can define the structure and dynamics of a wide range of biological models in a fully machine readable format. We describe how LEMS underpins the latest version of NeuroML and show that this framework can define models of ion channels, synapses, neurons and networks. Unit handling, often a source of error when reusing models, is built into the core of the language by specifying physical quantities in models in terms of the base dimensions. We show how LEMS, together with the open source Java and Python based libraries we have developed, facilitates the generation of scripts for multiple neuronal simulators and provides a route for simulator free code generation. We establish that LEMS can be used to define models from systems biology and map them to neuroscience-domain specific simulators, enabling models to be shared between these traditionally separate disciplines. LEMS and NeuroML 2 provide a new, comprehensive framework for defining computational models of neuronal and other biological systems in a machine readable format, making them more reproducible and increasing the transparency and accessibility of their underlying structure and properties.},
author = {Cannon, Robert C. and Gleeson, Padraig and Crook, Sharon and Ganapathy, Gautham and Marin, Boris and Piasini, Eugenio and Silver, R. Angus},
doi = {10.3389/fninf.2014.00079},
file = {:home/michiel/Downloads/fninf-08-00079.pdf:pdf},
issn = {16625196},
journal = {Frontiers in Neuroinformatics},
keywords = {Model description language,Model sharing,Simulation,Spiking neural networks,Standardization},
number = {SEP},
pages = {1--21},
title = {{LEMS: A language for expressing complex biological models in concise and hierarchical form and its use in underpinning NeuroML 2}},
volume = {8},
year = {2014}
}

@article{PyRates,
    author = {Gast, Richard AND Rose, Daniel AND Salomon, Christoph AND Möller, Harald E. AND Weiskopf, Nikolaus AND Knösche, Thomas R.},
    journal = {PLOS ONE},
    publisher = {Public Library of Science},
    title = {PyRates—A Python framework for rate-based neural simulations},
    year = {2019},
    month = {12},
    volume = {14},
    url = {https://doi.org/10.1371/journal.pone.0225900},
    pages = {1-26},
    abstract = {In neuroscience, computational modeling has become an important source of insight into brain states and dynamics. A basic requirement for computational modeling studies is the availability of efficient software for setting up models and performing numerical simulations. While many such tools exist for different families of neural models, there is a lack of tools allowing for both a generic model definition and efficiently parallelized simulations. In this work, we present PyRates, a Python framework that provides the means to build a large variety of rate-based neural models. PyRates provides intuitive access to and modification of all mathematical operators in a graph, thus allowing for a highly generic model definition. For computational efficiency and parallelization, the model is translated into a compute graph. Using the example of two different neural models belonging to the family of rate-based population models, we explain the mathematical formalism, software structure and user interfaces of PyRates. We show via numerical simulations that the behavior of the PyRates model implementations is consistent with the literature. Finally, we demonstrate the computational capacities and scalability of PyRates via a number of benchmark simulations of neural networks differing in size and connectivity.},
    number = {12},
    doi = {10.1371/journal.pone.0225900}
}

@article{fasttvb,
abstract = {The Virtual Brain (TVB) is now available as open-source cloud ecosystem on EBRAINS, a shared digital research platform for brain science. It offers services for constructing, simulating and analysing brain network models (BNMs) including the TVB network simulator; magnetic resonance imaging (MRI) processing pipelines to extract structural and functional connectomes; multiscale co-simulation of spiking and large-scale networks; a domain specific language for automatic high-performance code generation from user-specified models; simulation-ready BNMs of patients and healthy volunteers; Bayesian inference of epilepsy spread; data and code for mouse brain simulation; and extensive educational material. TVB cloud services facilitate reproducible online collaboration and discovery of data assets, models, and software embedded in scalable and secure workflows, a precondition for research on large cohort data sets, better generalizability and clinical translation.},
archivePrefix = {arXiv},
arxivId = {2102.05888},
author = {Schirner, Michael and Domide, Lia and Perdikis, Dionysios and Triebkorn, Paul and Stefanovski, Leon and Pai, Roopa and Popa, Paula and Valean, Bogdan and Palmer, Jessica and Langford, Chlo{\^{e}} and Blickensd{\"{o}}rfer, Andr{\'{e}} and van der Vlag, Michiel and Diaz-Pier, Sandra and Peyser, Alexander and Klijn, Wouter and Pleiter, Dirk and Nahm, Anne and Schmid, Oliver and Woodman, Marmaduke and Zehl, Lyuba and Fousek, Jan and Petkoski, Spase and Kusch, Lionel and Hashemi, Meysam and Marinazzo, Daniele and Mangin, Jean-Fran{\c{c}}ois and Fl{\"{o}}el, Agnes and Akintoye, Simisola and Stahl, Bernd Carsten and Cepic, Michael and Johnson, Emily and Deco, Gustavo and McIntosh, Anthony R. and Hilgetag, Claus C. and Morgan, Marc and Schuller, Bernd and Upton, Alex and McMurtrie, Colin and Dickscheid, Timo and Bjaalie, Jan G. and Amunts, Katrin and Mersmann, Jochen and Jirsa, Viktor and Ritter, Petra},
eprint = {2102.05888},
file = {:home/michiel/Downloads/2102.05888.pdf:pdf},
title = {{Brain Modelling as a Service: The Virtual Brain on EBRAINS}},
url = {http://arxiv.org/abs/2102.05888},
year = {2021}
}

@article{Montbrio2015,
abstract = {A major goal of neuroscience, statistical physics, and nonlinear dynamics is to understand how brain function arises from the collective dynamics of networks of spiking neurons. This challenge has been chiefly addressed through large-scale numerical simulations. Alternatively, researchers have formulated mean-field theories to gain insight into macroscopic states of large neuronal networks in terms of the collective firing activity of the neurons, or the firing rate. However, these theories have not succeeded in establishing an exact correspondence between the firing rate of the network and the underlying microscopic state of the spiking neurons. This has largely constrained the range of applicability of such macroscopic descriptions, particularly when trying to describe neuronal synchronization. Here, we provide the derivation of a set of exact macroscopic equations for a network of spiking neurons. Our results reveal that the spike generation mechanism of individual neurons introduces an effective coupling between two biophysically relevant macroscopic quantities, the firing rate and the mean membrane potential, which together govern the evolution of the neuronal network. The resulting equations exactly describe all possible macroscopic dynamical states of the network, including states of synchronous spiking activity. Finally, we show that the firing-rate description is related, via a conformal map, to a low-dimensional description in terms of the Kuramoto order parameter, called Ott-Antonsen theory. We anticipate that our results will be an important tool in investigating how large networks of spiking neurons self-organize in time to process and encode information in the brain.},
archivePrefix = {arXiv},
arxivId = {1506.06581},
author = {Montbri{\'{o}}, Ernest and Paz{\'{o}}, Diego and Roxin, Alex},
doi = {10.1103/PhysRevX.5.021028},
eprint = {1506.06581},
file = {:home/michiel/Downloads/PhysRevX.5.021028.pdf:pdf},
issn = {21603308},
journal = {Physical Review X},
keywords = {biological physics,interdisciplinary physics},
number = {2},
pages = {1--15},
title = {{Macroscopic description for networks of spiking neurons}},
volume = {5},
year = {2015}
}


@article{MLart2018,
abstract = {Advances in experimental techniques and computational power allowing researchers to gather anatomical and electrophysiological data at unprecedented levels of detail have fostered the development of increasingly complex models in computational neuroscience. Large-scale, biophysically detailed cell models pose a particular set of computational challenges, and this has led to the development of a number of domain-specific simulators. At the other level of detail, the ever growing variety of point neuron models increases the implementation barrier even for those based on the relatively simple integrate-and-fire neuron model. Independently of the model complexity, all modeling methods crucially depend on an efficient and accurate transformation of mathematical model descriptions into efficiently executable code. Neuroscientists usually publish model descriptions in terms of the mathematical equations underlying them. However, actually simulating them requires they be translated into code. This can cause problems because errors may be introduced if this process is carried out by hand, and code written by neuroscientists may not be very computationally efficient. Furthermore, the translated code might be generated for different hardware platforms, operating system variants or even written in different languages and thus cannot easily be combined or even compared. Two main approaches to addressing this issues have been followed. The first is to limit users to a fixed set of optimized models, which limits flexibility. The second is to allow model definitions in a high level interpreted language, although this may limit performance. Recently, a third approach has become increasingly popular: using code generation to automatically translate high level descriptions into efficient low level code to combine the best of previous approaches. This approach also greatly enriches efforts to standardize simulator-independent model description languages. In the past few years, a number of code generation pipelines have been developed in the computational neuroscience community, which differ considerably in aim, scope and functionality. This article provides an overview of existing pipelines currently used within the community and contrasts their capabilities and the technologies and concepts behind them.},
author = {Blundell, Inga and Brette, Romain and Cleland, Thomas A and Close, Thomas G and Coca, Daniel and Davison, Andrew P and Diaz-Pier, Sandra and {Fernandez Musoles}, Carlos and Gleeson, Padraig and Goodman, Dan F M and Hines, Michael and Hopkins, Michael W and Kumbhar, Pramod and Lester, David R and Marin, B{\'{o}}ris and Morrison, Abigail and M{\"{u}}ller, Eric and Nowotny, Thomas and Peyser, Alexander and Plotnikov, Dimitri and Richmond, Paul and Rowley, Andrew and Rumpe, Bernhard and Stimberg, Marcel and Stokes, Alan B and Tomkins, Adam and Trensch, Guido and Woodman, Marmaduke and Eppler, Jochen Martin},
doi = {10.3389/fninf.2018.00068},
issn = {1662-5196},
journal = {Frontiers in Neuroinformatics},
pages = {68},
title = {{Code Generation in Computational Neuroscience: A Review of Tools and Techniques}},
url = {https://www.frontiersin.org/article/10.3389/fninf.2018.00068},
volume = {12},
year = {2018}
}

@ARTICLE{Rabuffo2021,
  title    = "Neuronal cascades shape whole-brain functional dynamics at rest",
  author   = "Rabuffo, Giovanni and Fousek, Jan and Bernard, Christophe and Jirsa, Viktor",
  journal  = "eNeuro",
  month    =  sep,
  year     =  2021,
  url      = "http://dx.doi.org/10.1523/ENEURO.0283-21.2021",
  keywords = "EEG/fMRI; Neuronal Cascades; network modeling; resting state",
  issn     = "2373-2822",
  pmid     = "34583933",
  doi      = "10.1523/ENEURO.0283-21.2021"
}

@software{subramoney_anand_2019_2590760,
  author       = {Subramoney, Anand and
                  Diaz-Pier, Sandra and
                  Rao, Arjun and
                  Scherr, Franz and
                  Salaj, Darjan and
                  Bohnstingl, Thomas and
                  Jordan, Jakob and
                  Kopp, Nikolaus and
                  Hackhofer, Daniel and
                  Stekovic, Sinisa},
  title        = {IGITUGraz/L2L: v1.0.0-beta},
  month        = mar,
  year         = 2019,
  publisher    = {Zenodo},
  version      = {v1.0.0-beta},
  doi          = {10.5281/zenodo.2590760},
  url          = {https://doi.org/10.5281/zenodo.2590760}
}

@misc{peyser2019linking,
  title={Linking experimental and computational connectomics},
  author={Peyser, Alexander and Diaz Pier, Sandra and Klijn, Wouter and Morrison, Abigail and Triesch, Jochen},
  year={2019},
  publisher={MIT Press One Rogers Street, Cambridge, MA 02142-1209, USA journals-info~…}
}

@article{nakagawa2013bottom,
  title={Bottom up modeling of the connectome: linking structure and function in the resting brain and their changes in aging},
  author={Nakagawa, Tristan T and Jirsa, Viktor K and Spiegler, Andreas and McIntosh, Anthony R and Deco, Gustavo},
  journal={Neuroimage},
  volume={80},
  pages={318--329},
  year={2013},
  publisher={Elsevier}
}

@article{deco2014identification,
  title={Identification of optimal structural connectivity using functional connectivity and neural modeling},
  author={Deco, Gustavo and McIntosh, Anthony R and Shen, Kelly and Hutchison, R Matthew and Menon, Ravi S and Everling, Stefan and Hagmann, Patric and Jirsa, Viktor K},
  journal={Journal of Neuroscience},
  volume={34},
  number={23},
  pages={7910--7916},
  year={2014},
  publisher={Soc Neuroscience}
}

@article{falcon2016new,
  title={A new neuroinformatics approach to personalized medicine in neurology: The Virtual Brain},
  author={Falcon, Maria I and Jirsa, Viktor and Solodkin, Ana},
  journal={Current opinion in neurology},
  volume={29},
  number={4},
  pages={429},
  year={2016},
  publisher={NIH Public Access}
}

@article{einevoll2019scientific,
  title={The scientific case for brain simulations},
  author={Einevoll, Gaute T and Destexhe, Alain and Diesmann, Markus and Gr{\"u}n, Sonja and Jirsa, Viktor and de Kamps, Marc and Migliore, Michele and Ness, Torbj{\o}rn V and Plesser, Hans E and Sch{\"u}rmann, Felix},
  journal={Neuron},
  volume={102},
  number={4},
  pages={735--744},
  year={2019},
  publisher={Elsevier}
}

@article{lynn2019physics,
  title={The physics of brain network structure, function and control},
  author={Lynn, Christopher W and Bassett, Danielle S},
  journal={Nature Reviews Physics},
  volume={1},
  number={5},
  pages={318--332},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{bansal2018personalized,
  title={Personalized brain network models for assessing structure--function relationships},
  author={Bansal, Kanika and Nakuci, Johan and Muldoon, Sarah Feldt},
  journal={Current Opinion in Neurobiology},
  volume={52},
  pages={42--47},
  year={2018},
  publisher={Elsevier}
}

@article{hashemi2020bayesian,
  title={The Bayesian Virtual Epileptic Patient: A probabilistic framework designed to infer the spatial map of epileptogenicity in a personalized large-scale brain model of epilepsy spread},
  author={Hashemi, Meysam and Vattikonda, AN and Sip, V and Guye, Maxime and Bartolomei, Fabrice and Woodman, Michael Marmaduke and Jirsa, Viktor K},
  journal={NeuroImage},
  volume={217},
  pages={116839},
  year={2020},
  publisher={Elsevier}
}

@misc{cuda,
  author={NVIDIA and Vingelmann, Péter and Fitzek, Frank H.P.},
  title={CUDA, release: 10.2.89},
  year={2020},
  url={https://developer.nvidia.com/cuda-toolkit},
}

@article{jirsa2014nature,
  title={On the nature of seizure dynamics},
  author={Jirsa, Viktor K and Stacey, William C and Quilichini, Pascale P and Ivanov, Anton I and Bernard, Christophe},
  journal={Brain},
  volume={137},
  number={8},
  pages={2210--2230},
  year={2014},
  publisher={Oxford University Press}
}

@article{kuramoto1975international,
  title={International symposium on mathematical problems in theoretical physics},
  author={Kuramoto, Yoshiki},
  journal={Lecture notes in Physics},
  volume={30},
  pages={420},
  year={1975}
}

@article{wong2006recurrent,
  title={A recurrent network mechanism of time integration in perceptual decisions},
  author={Wong, Kong-Fatt and Wang, Xiao-Jing},
  journal={Journal of Neuroscience},
  volume={26},
  number={4},
  pages={1314--1328},
  year={2006},
  publisher={Soc Neuroscience}
}

@article{van2020exploring,
  title={Exploring Complex Brain-Simulation Workloads on Multi-GPU Deployments.},
  author={van der Vlag, Michiel A and Smaragdos, Georgios and Al-Ars, Zaid and Strydis, Christos},
  journal={ACM Trans. Archit. Code Optim.},
  volume={16},
  number={4},
  pages={53--1},
  year={2020}
}

@inproceedings{schemmel2010wafer,
  title={A wafer-scale neuromorphic hardware system for large-scale neural modeling},
  author={Schemmel, Johannes and Br{\"u}derle, Daniel and Gr{\"u}bl, Andreas and Hock, Matthias and Meier, Karlheinz and Millner, Sebastian},
  booktitle={2010 IEEE International Symposium on Circuits and Systems (ISCAS)},
  pages={1947--1950},
  year={2010},
  organization={IEEE}
}

@INPROCEEDINGS{
    arbor2019,
    author={N. {Abi Akar} and B. {Cumming} and V. {Karakasis} and A. {Küsters} and W. {Klijn} and A. {Peyser} and S. {Yates}},
    booktitle={2019 27th Euromicro International Conference on Parallel, Distributed and Network-Based Processing (PDP)},
    title={{Arbor --- A Morphologically-Detailed Neural Network Simulation Library for Contemporary High-Performance Computing Architectures}},
    year={2019}, month={feb}, volume={}, number={},
    pages={274--282},
    doi={10.1109/EMPDP.2019.8671560},
    ISSN={2377-5750}}

@article{furber2012overview,
  title={Overview of the spinnaker system architecture},
  author={Furber, Steve B and Lester, David R and Plana, Luis A and Garside, Jim D and Painkras, Eustace and Temple, Steve and Brown, Andrew D},
  journal={IEEE Transactions on Computers},
  volume={62},
  number={12},
  pages={2454--2467},
  year={2012},
  publisher={IEEE}
}

@article{fox2007spontaneous,
  title={Spontaneous fluctuations in brain activity observed with functional magnetic resonance imaging},
  author={Fox, Michael D and Raichle, Marcus E},
  journal={Nature reviews neuroscience},
  volume={8},
  number={9},
  pages={700--711},
  year={2007},
  publisher={Nature Publishing Group}
}

@misc{tensorflow2015-whitepaper,
title={ {TensorFlow}: Large-Scale Machine Learning on Heterogeneous Systems},
url={https://www.tensorflow.org/},
note={Software available from tensorflow.org},
author={
    Mart\'{\i}n~Abadi and
    Ashish~Agarwal and
    Paul~Barham and
    Eugene~Brevdo and
    Zhifeng~Chen and
    Craig~Citro and
    Greg~S.~Corrado and
    Andy~Davis and
    Jeffrey~Dean and
    Matthieu~Devin and
    Sanjay~Ghemawat and
    Ian~Goodfellow and
    Andrew~Harp and
    Geoffrey~Irving and
    Michael~Isard and
    Yangqing Jia and
    Rafal~Jozefowicz and
    Lukasz~Kaiser and
    Manjunath~Kudlur and
    Josh~Levenberg and
    Dandelion~Man\'{e} and
    Rajat~Monga and
    Sherry~Moore and
    Derek~Murray and
    Chris~Olah and
    Mike~Schuster and
    Jonathon~Shlens and
    Benoit~Steiner and
    Ilya~Sutskever and
    Kunal~Talwar and
    Paul~Tucker and
    Vincent~Vanhoucke and
    Vijay~Vasudevan and
    Fernanda~Vi\'{e}gas and
    Oriol~Vinyals and
    Pete~Warden and
    Martin~Wattenberg and
    Martin~Wicke and
    Yuan~Yu and
    Xiaoqiang~Zheng},
  year={2015},
}

@article{GeNN,
abstract = {Large-scale numerical simulations of detailed brain circuit models are important for identifying hypotheses on brain functions and testing their consistency and plausibility. An ongoing challenge for simulating realistic models is, however, computational speed. In this paper, we present the GeNN (GPU-enhanced Neuronal Networks) framework, which aims to facilitate the use of graphics accelerators for computational models of large-scale neuronal networks to address this challenge. GeNN is an open source library that generates code to accelerate the execution of network simulations on NVIDIA GPUs, through a flexible and extensible interface, which does not require in-depth technical knowledge from the users. We present performance benchmarks showing that 200-fold speedup compared to a single core of a CPU can be achieved for a network of one million conductance based Hodgkin-Huxley neurons but that for other models the speedup can differ. GeNN is available for Linux, Mac OS X and Windows platforms. The source code, user manual, tutorials, Wiki, in-depth example projects and all other related information can be found on the project website http://genn-team.github.io/genn/.},
author = {Yavuz, Esin and Turner, James and Nowotny, Thomas},
doi = {10.1038/srep18854},
file = {:home/michiel/Documents/Atrticles/rateML/srep18854.pdf:pdf},
issn = {20452322},
journal = {Scientific Reports},
month = {jan},
pages = {18854},
pmid = {26740369},
publisher = {The Author(s)},
title = {{GeNN: A code generation framework for accelerated brain simulations}},
url = {http://dx.doi.org/10.1038/srep18854 http://10.0.4.14/srep18854 https://www.nature.com/articles/srep18854#supplementary-information},
volume = {6},
year = {2016}
}

@article{Stimberg2019,
    title = {Brian 2, an intuitive and efficient neural simulator},
    volume = {8},
    issn = {2050-084X},
    doi = {10.7554/eLife.47314},
    journal = {eLife},
    author = {Stimberg, Marcel and Brette, Romain and Goodman, Dan FM},
    editor = {Skinner, Frances K},
    month = aug,
    year = {2019},
    pages = {e47314}
}

@inproceedings{mci/Plotnikov2016,
author = {Plotnikov, Dimitri AND Blundell, Inga AND Ippen, Tammo AND Eppler, Jochen Martin AND Morrison, Abigail AND Rumpe, Bernhard},
title = {NESTML: a modeling language for spiking neurons},
booktitle = {Modellierung 2016},
year = {2016},
editor = {Oberweis, Andreas AND Reussner, Ralf} ,
pages = { 93-108 },
publisher = {Gesellschaft für Informatik e.V.},
address = {Bonn}
}

@Inbook{Davison2013,
author={Davison, Andrew},
editor={Jaeger, Dieter and Jung, Ranu},
title="NineML",
bookTitle="Encyclopedia of Computational Neuroscience",
year="2013",
publisher="Springer New York",
address="New York, NY",
pages="1--2",
isbn="978-1-4614-7320-6",
doi="10.1007/978-1-4614-7320-6_375-2",
url="https://doi.org/10.1007/978-1-4614-7320-6_375-2"
}

@Article{         harris2020array,
 title         = {Array programming with {NumPy}},
 author        = {Charles R. Harris and K. Jarrod Millman and St{\'{e}}fan J.
                 van der Walt and Ralf Gommers and Pauli Virtanen and David
                 Cournapeau and Eric Wieser and Julian Taylor and Sebastian
                 Berg and Nathaniel J. Smith and Robert Kern and Matti Picus
                 and Stephan Hoyer and Marten H. van Kerkwijk and Matthew
                 Brett and Allan Haldane and Jaime Fern{\'{a}}ndez del
                 R{\'{i}}o and Mark Wiebe and Pearu Peterson and Pierre
                 G{\'{e}}rard-Marchant and Kevin Sheppard and Tyler Reddy and
                 Warren Weckesser and Hameer Abbasi and Christoph Gohlke and
                 Travis E. Oliphant},
 year          = {2020},
 month         = sep,
 journal       = {Nature},
 volume        = {585},
 number        = {7825},
 pages         = {357--362},
 doi           = {10.1038/s41586-020-2649-2},
 publisher     = {Springer Science and Business Media {LLC}},
 url           = {https://doi.org/10.1038/s41586-020-2649-2}
}

@misc{Curand,
author = {NVIDIA, Corporation},
journal = {NVIDIA Corporation, Santa Clara, California},
title = {CURAND library},
url = {http://scholar.google.com/scholar?hl=en&btnG=Search&q=intitle:CURAND+Library#0},
year = {2008}
}

@article{molder2021sustainable,
  title={Sustainable data analysis with Snakemake},
  author={M{\"o}lder, Felix and Jablonski, Kim Philipp and Letcher, Brice and Hall, Michael B and Tomkins-Tinch, Christopher H and Sochat, Vanessa and Forster, Jan and Lee, Soohyun and Twardziok, Sven O and Kanitz, Alexander and others},
  journal={F1000Research},
  volume={10},
  year={2021},
  publisher={Faculty of 1000 Ltd}
}

@article{CABRAL2011130,
title = {Role of local network oscillations in resting-state functional connectivity},
journal = {NeuroImage},
volume = {57},
number = {1},
pages = {130-139},
year = {2011},
issn = {1053-8119},
doi = {https://doi.org/10.1016/j.neuroimage.2011.04.010},
url = {https://www.sciencedirect.com/science/article/pii/S1053811911003880},
author = {Joana Cabral and Etienne Hugues and Olaf Sporns and Gustavo Deco},
keywords = {Resting state, Network oscillations, Modeling, Structural connectivity, Functional connectivity, Default-mode network},
abstract = {Spatio-temporally organized low-frequency fluctuations (<0.1Hz), observed in BOLD fMRI signal during rest, suggest the existence of underlying network dynamics that emerge spontaneously from intrinsic brain processes. Furthermore, significant correlations between distinct anatomical regions—or functional connectivity (FC)—have led to the identification of several widely distributed resting-state networks (RSNs). This slow dynamics seems to be highly structured by anatomical connectivity but the mechanism behind it and its relationship with neural activity, particularly in the gamma frequency range, remains largely unknown. Indeed, direct measurements of neuronal activity have revealed similar large-scale correlations, particularly in slow power fluctuations of local field potential gamma frequency range oscillations. To address these questions, we investigated neural dynamics in a large-scale model of the human brain's neural activity. A key ingredient of the model was a structural brain network defined by empirically derived long-range brain connectivity together with the corresponding conduction delays. A neural population, assumed to spontaneously oscillate in the gamma frequency range, was placed at each network node. When these oscillatory units are integrated in the network, they behave as weakly coupled oscillators. The time-delayed interaction between nodes is described by the Kuramoto model of phase oscillators, a biologically-based model of coupled oscillatory systems. For a realistic setting of axonal conduction speed, we show that time-delayed network interaction leads to the emergence of slow neural activity fluctuations, whose patterns correlate significantly with the empirically measured FC. The best agreement of the simulated FC with the empirically measured FC is found for a set of parameters where subsets of nodes tend to synchronize although the network is not globally synchronized. Inside such clusters, the simulated BOLD signal between nodes is found to be correlated, instantiating the empirically observed RSNs. Between clusters, patterns of positive and negative correlations are observed, as described in experimental studies. These results are found to be robust with respect to a biologically plausible range of model parameters. In conclusion, our model suggests how resting-state neural activity can originate from the interplay between the local neural dynamics and the large-scale structure of the brain.}
}

@article{Klockner2012,
abstract = {A common lament in the field of scientific computing concerns the ever-widening gap between hypothetical machine capabilities and the effort an individual programmer is able to spend to move a computational application towards exploiting a machine to the full extent of its capability. More sophisticated tools, compilers, and libraries are generally hoped to level this field, enabling users to achieve good results even with modest investment. PyCUDA is a contribution to the tools for graphics processing unit (GPU) computing. PyCUDA has a two-fold aim. First, it aims to simplify the usage of existing basic concepts of CUDA C. Importantly, it does not attempt to change or reinvent the basic notions of GPU programming, but instead, as a foundation for further tools, just exposes them as is through a carefully engineered interface. Key features of this interface include generous use of sensible defaults, automatic error checking, and automatic resource management. Second, and strictly on top of the first, basic layer, PyCUDA provides abstractions that support a number of very common usage patterns involving a GPU equivalent of NumPy arrays. Although PyCUDA gives the user access to a compiled language (CUDA C), it attempts to avoid the development iteration penalty commonly associated with compiled languages, instead retaining the satisfaction and immediacy of scripting. PyCUDA and PyOpenCL, as open-source projects, thrive on user feedback, particularly feedback regarding limitations, bugs, or missing features that users encounter. {\textcopyright} 2012 Elsevier Inc. All rights reserved.},
archivePrefix = {arXiv},
arxivId = {1304.5553},
author = {Kl{\"{o}}ckner, Andreas and Pinto, Nicolas and Catanzaro, Bryan and Lee, Yunsup and Ivanov, Paul and Fasih, Ahmed},
doi = {10.1016/B978-0-12-385963-1.00027-7},
eprint = {1304.5553},
file = {:home/michiel/Downloads/1304.5553.pdf:pdf},
isbn = {9780123859631},
journal = {GPU Computing Gems Jade Edition},
pages = {373--385},
title = {{GPU Scripting and Code Generation with PyCUDA}},
year = {2012}
}
@article{Ott2008,
abstract = {It is shown that, in the infinite size limit, certain systems of globally coupled  phase oscillators display low dimensional dynamics. In particular, we derive an explicit finite set of nonlinear ordinary differential equations for the macroscopic evolution of the systems considered. For example, an exact, closed form solution for the nonlinear time evolution of the Kuramoto problem with a Lorentzian oscillator frequency distribution function is obtained. Low dimensional behavior is also demonstrated for several prototypical extensions of the Kuramoto model, and time-delayed coupling is also considered.},
author = {Ott, Edward and Antonsen, Thomas M},
doi = {10.1063/1.2930766},
issn = {1089-7682 (Electronic)},
journal = {Chaos (Woodbury, N.Y.)},
keywords = {Algorithms,Biological Clocks,Computer Simulation,Feedback,Metabolic Networks and Pathways,Models, Theoretical,Nerve Net,Nonlinear Dynamics,Oscillometry,methods,physiology},
month = {sep},
number = {3},
pages = {37113},
pmid = {19045487},
title = {{Low dimensional behavior of large systems of globally coupled oscillators.}},
volume = {18},
year = {2008}
}

@InProceedings{LattnerAdve:tutorial,
  author={Chris Lattner and Vikram Adve},
  title="{The LLVM Compiler Framework and Infrastructure Tutorial}",
  month={Sep},
  year={2004},
  address={West Lafayette, Indiana},
  booktitle="{LCPC'04 Mini Workshop on Compiler Research Infrastructures}"
}

@article{rateml2022,
abstract={Whole brain network models are now an established tool in scientific and clinical research, however their use in a larger workflow still adds significant informatics complexity. We propose a tool, RateML, that enables users to generate such models from a succinct declarative description, in which the mathematics of the model are described without specifying how their simulation should be implemented. RateML builds on NeuroML’s Low Entropy Model Specification (LEMS), an XML based language for specifying models of dynamical systems, allowing descriptions of neural mass and discretized neural field models, as implemented by the Virtual Brain (TVB) simulator: the end user describes their model’s mathematics once and generates and runs code for different languages, targeting both CPUs for fast single simulations and GPUs for parallel ensemble simulations. High performance parallel simulations are crucial for tuning many parameters of a model to empirical data such as functional magnetic resonance imaging (fMRI), with reasonable execution times on small or modest hardware resources. Specifically, while RateML can generate Python model code, it enables generation of Compute Unified Device Architecture C++ code for NVIDIA GPUs. When a CUDA implementation of a model is generated, a tailored model driver class is produced, enabling the user to tweak the driver by hand and perform the parameter sweep. The model and driver can be executed on any compute capable NVIDIA GPU with a high degree of parallelization, either locally or in a compute cluster environment. The results reported in this manuscript show that with the CUDA code generated by RateML, it is possible to explore thousands of parameter combinations with a single Graphics Processing Unit for different models, substantially reducing parameter exploration times and resource usage for the brain network models, in turn accelerating the research workflow itself. This provides a new tool to create efficient and broader parameter fitting workflows, support studies on larger cohorts, and derive more robust and statistically relevant conclusions about brain dynamics.},
author={van der Vlag, Michiel and Woodman, Marmaduke and Fousek, Jan and Diaz-Pier, Sandra and Pérez Martín, Aarón and Jirsa, Viktor and Morrison, Abigail},
title={RateML: A Code Generation Tool for Brain Network Models},      
journal={Frontiers in Network Physiology},      
volume={2},           
year={2022},        
url={https://www.frontiersin.org/articles/10.3389/fnetp.2022.826345},       
doi={10.3389/fnetp.2022.826345},      
issn={2674-0109}  
}

@ARTICLE{Goldman2023,
  
AUTHOR={Goldman, Jennifer S. and Kusch, Lionel and Aquilue, David and Yalçınkaya, Bahar Hazal and Depannemaecker, Damien and Ancourt, Kevin and Nghiem, Trang-Anh E. and Jirsa, Viktor and Destexhe, Alain},   
	 
TITLE={A comprehensive neural simulation of slow-wave sleep and highly responsive wakefulness dynamics},      
	
JOURNAL={Frontiers in Computational Neuroscience},      
	
VOLUME={16},           
	
YEAR={2023},      
	  
URL={https://www.frontiersin.org/articles/10.3389/fncom.2022.1058957},       
	
DOI={10.3389/fncom.2022.1058957},      
	
ISSN={1662-5188},   
   
ABSTRACT={Hallmarks of neural dynamics during healthy human brain states span spatial scales from neuromodulators acting on microscopic ion channels to macroscopic changes in communication between brain regions. Developing a scale-integrated understanding of neural dynamics has therefore remained challenging. Here, we perform the integration across scales using mean-field modeling of Adaptive Exponential (AdEx) neurons, explicitly incorporating intrinsic properties of excitatory and inhibitory neurons. The model was run using The Virtual Brain (TVB) simulator, and is open-access in EBRAINS. We report that when AdEx mean-field neural populations are connected via structural tracts defined by the human connectome, macroscopic dynamics resembling human brain activity emerge. Importantly, the model can qualitatively and quantitatively account for properties of empirically observed spontaneous and stimulus-evoked dynamics in space, time, phase, and frequency domains. Large-scale properties of cortical dynamics are shown to emerge from both microscopic-scale adaptation that control transitions between wake-like to sleep-like activity, and the organization of the human structural connectome; together, they shape the spatial extent of synchrony and phase coherence across brain regions consistent with the propagation of sleep-like spontaneous traveling waves at intermediate scales. Remarkably, the model also reproduces brain-wide, enhanced responsiveness and capacity to encode information particularly during wake-like states, as quantified using the perturbational complexity index. The model was run using The Virtual Brain (TVB) simulator, and is open-access in EBRAINS. This approach not only provides a scale-integrated understanding of brain states and their underlying mechanisms, but also open access tools to investigate brain responsiveness, toward producing a more unified, formal understanding of experimental data from conscious and unconscious states, as well as their associated pathologies.}
}

@article {Aquilu2023,
author = {David Aquilu{\'e}-Llorens and Jennifer S. Goldman and Alain Destexhe},
title = {High-density exploration of activity states in a multi-area brain model},
elocation-id = {2023.05.18.541285},
year = {2023},
doi = {10.1101/2023.05.18.541285},
publisher = {Cold Spring Harbor Laboratory},
abstract = {Biophysically-grounded whole-brain models were built recently using tractography data to interconnect multiple mesoscopic models, which can simulate the dynamics of neuronal populations with only a few equations. Mean-field models of neural populations, specifically the Adapting AdEx mean-field, was used for this purpose because it can integrate key biophysical mechanisms such as spike-frequency adaptation and its regulation at cellular scales, to the emergence of brain-scale dynamics. Using this approach, with the Virtual Brain (TVB) environment, it has been possible to model the macroscopic transitions between brain states, described by variation in brain-scale dynamics between asynchronous and rapid dynamics during conscious brain states, and synchronized slow-waves, with Up-and-Down state dynamics during unconscious brain states, emerging from mechanisms at the cellular level. Transitions between brain states are driven by changes in neuromodulation that can be due to intrinsic regulation during sleep-wake cycles or extrinsic factors such as anesthetics, which, in turn, affect spike-frequency adaptation. Here, we perform a dense grid parameter exploration of the TVB-AdEx model, making use of High Performance Computing, to thoroughly explore the properties of this model. We find that there is a remarkable robustness of the effect of adaptation to induce synchronized slow-wave activity. Moreover, the occurrence of slow waves is often paralleled with a closer relation between functional and structural connectivity. We find that hyperpolarization can also generate unconscious-like synchronized Up and Down states, which may be a mechanism underlying the action of anesthetics. We conclude that the parameter space of the TVB-AdEx model reveals features identified experimentally in sleep and anesthesia.Competing Interest StatementThe authors have declared no competing interest.},
URL = {https://www.biorxiv.org/content/early/2023/05/18/2023.05.18.541285},
eprint = {https://www.biorxiv.org/content/early/2023/05/18/2023.05.18.541285.full.pdf},
journal = {bioRxiv}
}

@article{divolo,
    author = {di Volo, Matteo and Romagnoni, Alberto and Capone, Cristiano and Destexhe, Alain},
    title = "{Biologically Realistic Mean-Field Models of Conductance-Based Networks of Spiking Neurons with Adaptation}",
    journal = {Neural Computation},
    volume = {31},
    number = {4},
    pages = {653-680},
    year = {2019},
    month = {04},
    abstract = "{Accurate population models are needed to build very large-scale neural models, but their derivation is difficult for realistic networks of neurons, in particular when nonlinear properties are involved, such as conductance-based interactions and spike-frequency adaptation. Here, we consider such models based on networks of adaptive exponential integrate-and-fire excitatory and inhibitory neurons. Using a master equation formalism, we derive a mean-field model of such networks and compare it to the full network dynamics. The mean-field model is capable of correctly predicting the average spontaneous activity levels in asynchronous irregular regimes similar to in vivo activity. It also captures the transient temporal response of the network to complex external inputs. Finally, the mean-field model is also able to quantitatively describe regimes where high- and low-activity states alternate (up-down state dynamics), leading to slow oscillations. We conclude that such mean-field models are biologically realistic in the sense that they can capture both spontaneous and evoked activity, and they naturally appear as candidates to build very large-scale models involving multiple brain areas.}",
    issn = {0899-7667},
    doi = {10.1162/neco_a_01173},
    url = {https://doi.org/10.1162/neco\_a\_01173},
    eprint = {https://direct.mit.edu/neco/article-pdf/31/4/653/1050655/neco\_a\_01173.pdf},
}

@article{neurolibCakan2021,
abstract = {neurolib is a computational framework for whole-brain modeling written in Python. It provides a set of neural mass models that represent the average activity of a brain region on a mesoscopic scale. In a whole-brain network model, brain regions are connected with each other based on biologically informed structural connectivity, i.e., the connectome of the brain. neurolib can load structural and functional datasets, set up a whole-brain model, manage its parameters, simulate it, and organize its outputs for later analysis. The activity of each brain region can be converted into a simulated BOLD signal in order to calibrate the model against empirical data from functional magnetic resonance imaging (fMRI). Extensive model analysis is made possible using a parameter exploration module, which allows one to characterize a model's behavior as a function of changing parameters. An optimization module is provided for fitting models to multimodal empirical data using evolutionary algorithms. neurolib is designed to be extendable and allows for easy implementation of custom neural mass models, offering a versatile platform for computational neuroscientists for prototyping models, managing large numerical experiments, studying the structure–function relationship of brain networks, and for performing in-silico optimization of whole-brain models.},
author = {Cakan, Caglar and Jajcay, Nikola and Obermayer, Klaus},
doi = {10.1007/s12559-021-09931-9},
file = {:home/michiel/Downloads/s12559-021-09931-9.pdf:pdf},
issn = {18669964},
journal = {Cognitive Computation},
keywords = {Brain networks,Neural mass model,Neuroinformatics,Whole-brain model},
pages = {1132--1152},
publisher = {Springer US},
title = {{neurolib: A Simulation Framework for Whole-Brain Neural Mass Modeling}},
url = {https://doi.org/10.1007/s12559-021-09931-9},
volume = {2},
year = {2021}
}

@ARTICLE{yegenoglu2022,
AUTHOR={Yegenoglu, Alper and Subramoney, Anand and Hater, Thorsten and Jimenez-Romero, Cristian and Klijn, Wouter and Pérez Martín, Aarón and van der Vlag, Michiel and Herty, Michael and Morrison, Abigail and Diaz-Pier, Sandra},   
TITLE={Exploring Parameter and Hyper-Parameter Spaces of Neuroscience Models on High Performance Computers With Learning to Learn},
JOURNAL={Frontiers in Computational Neuroscience},
VOLUME={16},           
YEAR={2022},
URL={https://www.frontiersin.org/articles/10.3389/fncom.2022.885207},
DOI={10.3389/fncom.2022.885207},
ISSN={1662-5188},
}

@article{domingo2017multimodal,
  title={Multimodal mechanistic signatures for neurodegenerative diseases (NeuroMMSig): a web server for mechanism enrichment},
  author={Domingo-Fern{\'a}ndez, Daniel and Kodamullil, Alpha Tom and Iyappan, Anandhi and Naz, Mufassra and Emon, Mohammad Asif and Raschka, Tamara and Karki, Reagon and Springstubbe, Stephan and Ebeling, Christian and Hofmann-Apitius, Martin},
  journal={Bioinformatics},
  volume={33},
  number={22},
  pages={3679--3681},
  year={2017},
  publisher={Oxford University Press}
}

@article{stefanovski2019linking,
  title={Linking molecular pathways and large-scale computational modeling to assess candidate disease mechanisms and pharmacodynamics in Alzheimer's disease},
  author={Stefanovski, Leon and Triebkorn, Paul and Spiegler, Andreas and Diaz-Cortes, Margarita-Arimatea and Solodkin, Ana and Jirsa, Viktor and McIntosh, Anthony Randal and Ritter, Petra and Alzheimer's Disease Neuroimaging Initiative},
  journal={Frontiers in computational neuroscience},
  volume={13},
  pages={54},
  year={2019},
  publisher={Frontiers Media SA}
}

@misc{sqlite2020hipp, 
  title={{SQLite}},
  url={https://www.sqlite.org/index.html},
  version={3.31.1},
  year={2020},
  author={Hipp, Richard D}
} 

@article{silva_pereira_effect_2017,
	title = {Effect of field spread on resting-state {MEG} functional network analysis: a computational modeling study},
	volume = {7},
	shorttitle = {Effect of field spread on resting-state {MEG} functional network analysis},
	doi = {10.1089/brain.2017.0525},
	abstract = {A popular way to analyze resting-state EEG and MEG data is to treat them as a functional network in which sensors are identified with nodes and the interaction between channel time-series with the network connections. Although conceptually appealing, the network-theoretical approach to sensor-level EEG and MEG data is challenged by the fact that EEG and MEG time-series are mixtures of source activity. It is therefore of interest to assess the relationship between functional networks of source activity and the ensuing sensor-level networks. Since these topological features are of high interest in experimental studies, we address the question of to what extent the network topology can be reconstructed from sensor-level functional connectivity measures in case of MEG data. Simple simulations that consider only a small number of regions do not allow to assess network properties; therefore, we use a diffusion MRI-constrained whole-brain computational model of resting-state activity. Our motivation lies behind the fact that still many contributions found in the literature perform network analysis at sensor level, and we aim at showing the discrepancies between source- and sensor-level network topologies using realistic simulations of resting-state cortical activity. Our main findings are that the effect of field spread on network topology depends on the type of interaction (instantaneous or lagged) and leads to an underestimation of lagged functional connectivity at sensor level due to instantaneous mixing of cortical signals, instantaneous interaction is more sensitive to field spread than lagged interaction, and discrepancies are reduced when using planar gradiometers rather than axial gradiometers. We therefore recommend to use lagged interaction measures on planar gradiometer data when investigating network properties of resting-state sensor-level MEG data.},
	journal = {Brain connectivity},
	author = {Silva Pereira, Silvana and Hindriks, Rikkert and Mühlberg, Stefanie and Maris, Eric and Ede, Freek and Griffa, Alessandra and Hagmann, Patrick and Deco, Gustavo},
	month = sep,
	year = {2017},
	file = {Full Text PDF:/home/kusch/Zotero/storage/PKZFAREM/Silva Pereira et al. - 2017 - Effect of field spread on resting-state MEG functi.pdf:application/pdf},
}

@article{Sazonov2009,
abstract = {The phase locking index (PLI) was introduced to quantify in a statistical sense the phase synchronization of two signals. It has been commonly used to process biosignals. In this article, we investigate the PLI for measuring the interdependency of cortical source signals (CSSs) recorded in the Electroencephalogram (EEG). To this end, we consider simple analytical models for the mapping of simulated CSSs into the EEG. For these models, the PLI is investigated analytically and through numerical simulations. An evaluation is made of the sensitivity of the PLI to the amount of crosstalk between the sources through biological tissues of the head. It is found that the PLI is a useful interdependency measure for CSSs, especially when the amount of crosstalk is small. Another common interdependency measure is the coherence. A direct comparison of both measures has not been made in the literature so far. We assess the performance of the PLI and coherence for estimation and detection purposes based on, respectively, a normalized variance and a novel statistical measure termed contrast. Based on these performance measures, it is found that the PLI is similar or better than the CM in most cases. This result is also confirmed through analysis of EEGs recorded from epileptic patients.},
author = {Sazonov, Andrei V. and Ho, Chin Keong and Bergmans, Jan W.M. and Arends, Johan B.A.M. and Griep, Paul A.M. and Verbitskiy, Evgeny A. and Cluitmans, Pierre J.M. and Boon, Paul A.J.M.},
doi = {10.1007/s00422-008-0283-4},
file = {:home/michiel/Documents/Articles/Analysis/422_2008_Article_283.pdf:pdf},
issn = {03401200},
journal = {Biological Cybernetics},
keywords = {Contrast,Correlation,Cortical sources,Coupling,Distribution function,EEG,Interdependency,Model,Phase locking},
number = {2},
pages = {129--146},
pmid = {19152066},
title = {{An investigation of the phase locking index for measuring of interdependency of cortical source signals recorded in the EEG}},
volume = {100},
year = {2009}
}

@article{STEPHAN2007387,
title = {Comparing hemodynamic models with DCM},
journal = {NeuroImage},
volume = {38},
number = {3},
pages = {387-401},
year = {2007},
issn = {1053-8119},
doi = {https://doi.org/10.1016/j.neuroimage.2007.07.040},
url = {https://www.sciencedirect.com/science/article/pii/S1053811907006489},
author = {Klaas Enno Stephan and Nikolaus Weiskopf and Peter M. Drysdale and Peter A. Robinson and Karl J. Friston},
keywords = {Dynamic causal modeling, Balloon model, Effective connectivity, BOLD signal, Bayesian model selection, System identification},
abstract = {The classical model of blood oxygen level-dependent (BOLD) responses by Buxton et al. [Buxton, R.B., Wong, E.C., Frank, L.R., 1998. Dynamics of blood flow and oxygenation changes during brain activation: the Balloon model. Magn. Reson. Med. 39, 855–864] has been very important in providing a biophysically plausible framework for explaining different aspects of hemodynamic responses. It also plays an important role in the hemodynamic forward model for dynamic causal modeling (DCM) of fMRI data. A recent study by Obata et al. [Obata, T., Liu, T.T., Miller, K.L., Luh, W.M., Wong, E.C., Frank, L.R., Buxton, R.B., 2004. Discrepancies between BOLD and flow dynamics in primary and supplementary motor areas: application of the Balloon model to the interpretation of BOLD transients. NeuroImage 21, 144–153] linearized the BOLD signal equation and suggested a revised form for the model coefficients. In this paper, we show that the classical and revised models are special cases of a generalized model. The BOLD signal equation of this generalized model can be reduced to that of the classical Buxton model by simplifying the coefficients or can be linearized to give the Obata model. Given the importance of hemodynamic models for investigating BOLD responses and analyses of effective connectivity with DCM, the question arises which formulation is the best model for empirically measured BOLD responses. In this article, we address this question by embedding different variants of the BOLD signal equation in a well-established DCM of functional interactions among visual areas. This allows us to compare the ensuing models using Bayesian model selection. Our model comparison approach had a factorial structure, comparing eight different hemodynamic models based on (i) classical vs. revised forms for the coefficients, (ii) linear vs. non-linear output equations, and (iii) fixed vs. free parameters, ε, for region-specific ratios of intra- and extravascular signals. Using fMRI data from a group of twelve subjects, we demonstrate that the best model is a non-linear model with a revised form for the coefficients, in which ε is treated as a free parameter.}
}


@article{brette_adaptive_2005,
	title = {Adaptive {Exponential} {Integrate}-and-{Fire} {Model} as an {Effective} {Description} of {Neuronal} {Activity}},
	volume = {94},
	issn = {0022-3077},
	url = {http://www.physiology.org/doi/10.1152/jn.00686.2005},
	doi = {10.1152/jn.00686.2005},
	abstract = {We introduce a two-dimensional integrate-and-fire model that combines an exponential spike mechanism with an adaptation equation, based on recent theoretical findings. We describe a systematic method to estimate its parameters with simple electrophysiological protocols (current-clamp injection of pulses and ramps) and apply it to a detailed conductance-based model of a regular spiking neuron. Our simple model predicts correctly the timing of 96\% of the spikes (±2 ms) of the detailed model in response to injection of noisy synaptic conductances. The model is especially reliable in high-conductance states, typical of cortical activity in vivo, in which intrinsic conductances were found to have a reduced role in shaping spike trains. These results are promising because this simple model has enough expressive power to reproduce qualitatively several electrophysiological classes described in vitro.},
	number = {5},
	urldate = {2018-02-15},
	journal = {Journal of Neurophysiology},
	author = {Brette, Romain and Gerstner, Wulfram},
	month = nov,
	year = {2005},
	pages = {3637--3642},
	file = {Full Text PDF:/home/kusch/Zotero/storage/UNMA9QRR/Brette and Gerstner - 2005 - Adaptive Exponential Integrate-and-Fire Model as a.pdf:application/pdf;Snapshot:/home/kusch/Zotero/storage/FENAKEFP/jn.00686.html:text/html},
}


@article{boustani_master_2009,
	title = {A {Master} {Equation} {Formalism} for {Macroscopic} {Modeling} of {Asynchronous} {Irregular} {Activity} {States}},
	language = {en},
	author = {El Boustani, Sami and Destexhe, Alain},
	year = {2009},
	keywords = {Neurons, Action Potentials, Animals, Cerebral Cortex, Computer Simulation, Linear Models, Models, Neurological, Neural Inhibition, Neural Networks (Computer), Time Factors, Wakefulness},
	pages = {55},
	file = {Boustani et Destexhe - A Master Equation Formalism for Macroscopic Modeli.pdf:/home/kusch/Zotero/storage/CNGFYG79/Boustani et Destexhe - A Master Equation Formalism for Macroscopic Modeli.pdf:application/pdf;Snapshot:/home/kusch/Zotero/storage/8NZQ6JXG/A-Master-Equation-Formalism-for-Macroscopic.html:text/html;Submitted Version:/home/kusch/Zotero/storage/YG426HB7/El Boustani and Destexhe - 2009 - A Master Equation Formalism for Macroscopic Modeli.pdf:application/pdf},
}

@article{Carlu2020,
  doi = {10.1152/jn.00399.2019},
  url = {https://doi.org/10.1152/jn.00399.2019},
  year = {2020},
  month = mar,
  publisher = {American Physiological Society},
  volume = {123},
  number = {3},
  pages = {1042--1051},
  author = {M. Carlu and O. Chehab and L. Dalla Porta and D. Depannemaecker and C. H{\'{e}}ric{\'{e}} and M. Jedynak and E. K\"{o}ksal Ers\"{o}z and P. Muratore and S. Souihel and C. Capone and Y. Zerlaut and A. Destexhe and M. di Volo},
  title = {A mean-field approach to the dynamics of networks of complex neurons,  from nonlinear Integrate-and-Fire to Hodgkin{\textendash}Huxley models},
  journal = {Journal of Neurophysiology}
}


